A Projection-Stable Grammatical Model for the Distributed Execution of Administrative Processes with Emphasis on Actors' Views

During the last two decades, the decentralized execution of business processes has been one of the main research topics in Business Process Management. Several models (languages) for processes' specification in order to facilitate their distributed execution, have been proposed. LSAWfP is among the most recent in this area: it helps to specify administrative processes with grammatical models indicating, in addition to their fundamental elements, the permissions (reading, writing and execution) of each actor in relation to each of their tasks. In this paper, we present a model for a completely decentralized and artifact-centric execution of administrative processes specified using LSAWfP. The presented model puts particular emphasis on actors' views: it then allows the confidential execution of certain tasks by ensuring that, each actor potentially has only a partial perception of the processes' global execution states. The model thus solves a very important problem in business process execution, which is often sidelined in existing approaches. To accomplish this, the model rely on three projection algorithms allowing to partially replicate the processes' global execution states at a given moment, to consistently update the obtained partial states and to deduce new coherent global states. The proposal of these three algorithms, the proof of underlying mathematical tools' stability and a proposal of their implementation, are this paper's main contributions.

==> p2ptinywfms.tex <==
\section{Expérimentation avec P2PTinyWfMS: un prototype expérimental de P2P-SGWf-View}
Les algorithmes présentés dans ce manuscrit, ont tous été codés en Haskell et en Java puis testés avec des résultats satisfaisants. En java, nous avons introduit ces algorithmes dans l'outil \textit{P2PTinyWfMS}.
Il s'agit d'un outil développé sous Eclipse\footnote{https://www.eclipse.org} et dédié à la simulation de l'exécution distribuée des workflows administratifs spécifiés à l'aide de notre LSPWfA. Conformément à l'architecture des P2P-SGWf-View (voir figure \ref{fig:architectureSimplifiePair} page \pageref{fig:architectureSimplifiePair}), \textit{P2PTinyWfMS} possède un front-end pour l'affichage et l'édition graphique des artefacts manipulés lors de l'exécution d'une procédure d'entreprise (voir figure \ref{p2ptinywfms-3}), ainsi qu'un module de communication  construit à partir de \textit{Shared-data Overlay Network (SON)}\footnote{SON (Shared-data Overlay Network) \cite{SON} est un middleware proposant plusieurs DSL (Domain Specific Language) pour faciliter la mise en oeuvre des systèmes P2P dont les composants communiquent par invocation de services. SON est disponible sous Eclipse à partir d'une famille de plugins SmartTools.} \cite{SON}. 

\begin{figure}[ht!]
    \centering
        \includegraphics[scale=0.22]{./images/p2ptinywfms-3.eps}
    \caption{Simulation de l'exécution du processus peer-review à l'aide de P2PTinyWfMS (site de l'éditeur associé).}
    \label{p2ptinywfms-3}
\end{figure}


